Knowledge Graph Fact Prediction via Knowledge-Enriched Tensor Factorization

We present a family of novel methods for embedding knowledge graphs into real-valued tensors. These tensor-based embeddings capture the ordered relations that are typical in the knowledge graphs represented by semantic web languages like RDF. Unlike many previous models, our methods can easily use prior background knowledge provided by users or extracted automatically from existing knowledge graphs. In addition to providing more robust methods for knowledge graph embedding, we provide a provably-convergent, linear tensor factorization algorithm. We demonstrate the efficacy of our models for the task of predicting new facts across eight different knowledge graphs, achieving between 5% and 50% relative improvement over existing state-of-the-art knowledge graph embedding techniques. Our empirical evaluation shows that all of the tensor decomposition models perform well when the average degree of an entity in a graph is high, with constraint-based models doing better on graphs with a small number of highly similar relations and regularization-based models dominating for graphs with relations of varying degrees of similarity.

==> tex_tables_image/acc_transitivity.tex <==
\begin{table*}
  \centering
  \renewcommand{\arraystretch}{1.4}
  \caption{Fact prediction performance using accuracy for all models. Linear + Reg is the linear tensor decomposition with regularization on $\te{R}$. Quad + Reg, our previous work \cite{padia2016inferring}, is the quadratic tensor decomposition with regularization on $\te{R}$. Linear + Constraint and Quad + Constraint are the linear and quadratic tensor decomposition with constraints on $\te{R}$ are incorporated as Lagrange model multiplier. Transitivity (the best similarity measure) is used as prior.}
    \begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
    \multicolumn{ 8}{|c|}{\textbf{Accuracy}} \\ \hline
\rowcolor{gray!15} \textbf{Model Name} & \textbf{Kinship} & \textbf{UMLS} & \textbf{WN18} & \textbf{FB13} & \textbf{DB10} & \textbf{Framenet} & \textbf{WN18RR} \\ \hline
\multicolumn{ 8}{|c|}{\textbf{Previous tensor factorization models}} \\ \hline
\textbf{RESCAL} & 80.62 & 68.26 & 42.18 & 45.08 & 40.16 & 61.5  & 44.42 \\\hline
\textbf{Non Negative RESCAL} & 78.15 & \textbf{68.69} & 63.62 & 58.43 & \textbf{48.73} & 60.88 & 45.22 \\\hline
\multicolumn{ 8}{|c|}{\textbf{Regularized/Constrained tensor factorization models}} \\ \hline
\textbf{Linear + Reg} & \textbf{81.54} & 68.04 & 60.31 & 57.96 & 47.93 & 54.75 & 46.06 \\\hline
\textbf{Quad + Reg} & 81.38 & 67.35 & 64.09 & 57.22 & 47.39 & 60.75 & 40 \\\hline
\textbf{Linear + Constraint} & 78.46 & 58.57 & 57.04 & 52.24 & 46.13 & 47    & 44.45 \\\hline
\textbf{Quad + Constraint} & 81.23 & 62    & \textbf{79.62} & \textbf{67.88} & 47.44 & \textbf{66.5} & \textbf{49.98} \\\hline
\end{tabular}%
  \label{acc_table}%
\end{table*}%
%\pagebreak

==> tex_tables_image/auc_transitivity.tex <==
\begin{table*}
  \centering
  \renewcommand{\arraystretch}{1.4}
  \caption{Fact prediction performance using Area Under the Curve (AUC) for all models. Linear + Reg is the linear tensor decomposition with regularization on $\te{R}$. Quad + Reg, our previous work \cite{padia2016inferring}, is the quadratic tensor decomposition with regularization on $\te{R}$. Linear + Constraint and Quad + Constraint are the linear and quadratic tensor decomposition with constraints on $\te{R}$ incorporated as a Lagrange multiplier. Transitivity (the best similarity measure) is used as prior.}
    \begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
\multicolumn{ 8}{|c|}{\textbf{Area Under Curve}} \\ \hline
\rowcolor{gray!15} \textbf{Model Name} & \textbf{Kinship} & \textbf{UMLS} & \textbf{WN18} & \textbf{FB13} & \textbf{DB10} & \textbf{Framenet} & \textbf{WN18RR} \\ \hline
\multicolumn{ 8}{|c|}{\textbf{Previous tensor factorization models}} \\ \hline
\textbf{RESCAL} & 93.24 & \textbf{88.53} & 62.13 & 65.37 & 61.27 & 82.54 & 66.63 \\ \hline
\textbf{Non Negative RESCAL} & 92.19 & 88.37 & 83.93 & 79.13 & 81.72 & 82.6 & 68.49\\ \hline
\multicolumn{ 8}{|c|}{\textbf{Regularized/Constrained tensor factorization models}} \\ \hline
    \textbf{Linear + Reg} & \textbf{93.99} & 88.22 & 81.86 & 80.07 & 80.79 & 78.11 & 69.15 \\ \hline
    \textbf{Quad + Reg} & 93.89 & 88.11 & 84.41 & 79.12 & 80.47 & 82.34 & 80 \\\hline
    \textbf{Linear + Constraint} & 92.87 & 84.71 & 80.18 & 75.79 & 80.67 & 73.64 & 66.46 \\\hline
    \textbf{Quad + Constraint} & 93.84 & 86.17 & \textbf{91.07} & \textbf{85.15} & 81.69 & \textbf{86.24} & \textbf{72.62} \\\hline
    \end{tabular}%
  \label{auc_table}%
\end{table*}

==> tex_tables_image/f1_macro_micro.tex <==
% Table generated by Excel2LaTeX from sheet 'f1_micro_macro'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|l|r|r|r|r|r|r|r|}
    \hline
    
    \textbf{f1 - macro (transitivity)} & \textbf{kinship} & \textbf{umls} & \textbf{WN18} & \textbf{FB13} & \textbf{DB10} & \textbf{Framenet} & \textbf{WN18RR} \\
    \hline
    \textbf{rescal} & 81.31 & 67.71 & 40.01 & 47.04 & 40    & 60.75 & 56.57 \\
    \hline
    \textbf{nn-r} & 77.23 & \textbf{69.43} & 63.69 & 58.28 & \textbf{47.73} & 60.75 & 52.35 \\
    \hline
    \textbf{linear + reg} & \textbf{81.54} & 68.04 & 60.31 & 57.96 & 47.39 & 54.75 & 47.58 \\
    \hline
    \textbf{quad + reg} & 81.38 & 67.35 & 64.09 & 57.22 & 47.39 & 60.62 & 44.92 \\
    \hline
    \textbf{linear + constraint} & 78.46 & 58.73 & 57.04 & 49.15 & 46.13 & 47    & 46.05 \\
    \hline
    \textbf{quad + constraint} & 81.23 & 62    & \textbf{79.62} & \textbf{67.88} & 44.13 & \textbf{66.5} & \textbf{68.01} \\
    \hline
    \end{tabular}%
  \label{tab:f1_macro}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'f1_micro_macro'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|l|r|r|r|r|r|r|r|}
    \hline
    \textbf{f1 - micro (transitivity)} & \textbf{kinship} & \textbf{umls} & \textbf{WN18} & \textbf{FB13} & \textbf{DB10} & \textbf{Framenet} & \textbf{WN18RR} \\
    \hline
    \textbf{rescal} & 74.54 & 51.85 & 3.01  & 18.53 & 0.41  & 41.23 & 40.45 \\
    \hline
    \textbf{nn-r} & 71.29 & \textbf{55.87} & 51.67 & 40.13 & \textbf{15.06} & 42.08 & 32.49 \\
    \hline
    \textbf{linear + reg} & \textbf{74.77} & 53.55 & 46.44 & 38.43 & 14.9  & 30.65 & 24.01 \\
    \hline
    \textbf{quad + reg} & 74.6  & 52.09 & 52.26 & 37.79 & 14.9  & 41.64 & 20.53 \\
    \hline
    \textbf{linear + constraint} & 71.5  & 37.55 & 42.62 & 27.9  & 10.86 & 23.07 & 26.82 \\
    \hline
    \textbf{quad + constraint} & 74.37 & 42.15 & \textbf{78.21} & \textbf{62.41} & 13.53 & \textbf{58.23} & \textbf{63.5} \\
    \hline
    \end{tabular}%
  \label{tab:f1_micro}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'f1_micro_macro'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|l|r|r|r|r|r|r|}
    \hline
          & \multicolumn{2}{c|}{\textbf{WN18}} & \multicolumn{2}{c|}{\textbf{FB13}} & \multicolumn{2}{c|}{\textbf{WN18RR}} \\
    \hline
          & \textbf{Macro} & \textbf{Micro} & \textbf{Macro} & \textbf{Micro} & \textbf{Macro} & \textbf{Micro} \\
    \hline
    \textbf{TransE} & 4.9   & 40.2  & 16.497 & 40.72 & 46.91 & 62.1 \\
    \hline
    \textbf{DistMult} & 49.67 & 49.96 & 29.2  & 53.76 & 37.76 & 61 \\
    \hline
    \textbf{Complex} & 52.187 & 50.52 & 28.86 & 54.06 & 34.235 & 60.88 \\
    \hline
    \textbf{Linear + Reg} & 53.364 & 64.84 & 35.4412 & 50.6  & 28.9497 & 48.9 \\
    \hline
    \textbf{Quad + Reg} & 58.092 & 57.7  & 34.8492 & 50.52 & 17.9626 & 48.5 \\
    \hline
    \textbf{Linear + Constraint} & 44.1  & 49.72 & 27.8226 & 44.72 & 26.9965 & 44.72 \\
    \hline
    \textbf{Quad + Constraint} & 85.6123 & 75.5  & 56.4785 & 59.04 & 59.09 & 62.54 \\
    \hline
    \end{tabular}%
  \label{tab:f1_macro_micro}%
\end{table}%




==> tex_tables_image/fb15k_237_table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Performance on FB15k dataset}
    \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{FB15k-237} & \textbf{AUC} & \textbf{F1-Micro} & \textbf{F1-Macro} \\
    \hline
    \textbf{Rescal} & 92.56 & 78.84 & 69.71 \\
    \hline
    \textbf{Non Negative Rescal} & 93.03 & 79.45 & 70.6 \\
    \hline
    \textbf{Linear + Reg} & 90    & 70.8  & 55.38 \\
    \hline
    \textbf{Quad + Reg} & 93.07 & 79.7  & 71.19 \\
    \hline
    \textbf{Linear + Constraint} & 81.88 & 13.7  & 46.8 \\
    \hline
    $\bigstar$  \quad \textbf{Quad + Constraint} & 86.47 & 59.59 & 36.63 \\
    \hline
    \end{tabular}%
  \label{tab:performance_fb15k}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Fact prediction evaluation of FB15\_237 by all systems and models}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    \textbf{Table 4 for fb15k\_237} & \textbf{AUC} & \textbf{F1-Micro} & \textbf{F1-Macro} & \textbf{ACC} \\
    \hline
    \textbf{Rescal} & 97.61 &  94.03 & 73.41 & 94.03 \\
    \hline
    \textbf{Non Negative Rescal} & 97.81  & 94.48 & 73.59 & 94.48 \\
    \hline
          &       &       &       &  \\
    \hline
    \textbf{TransE} & 50.84  & 41.11 & 4.21 & 41.12 \\
    \hline
    \textbf{DistMult} & 70.28  & 64.65& 45.33 & 64.65 \\
    \hline
    \textbf{Complex} & 67.64 & 61.59 & 35.12 & 61.59 \\
    \hline
          &       &       &       &  \\
    \hline
    \textbf{Linear + Reg} & 96.49 & 91.08  & 59.59 & 91.08 \\
    \hline
    \textbf{Quad + Reg} & 97.2    & 92.91 & 73.8 & 92.91 \\
    \hline
    \textbf{Linear + Constraint} & 80  & 43.53 & 1.06 & 43.53 \\
    \hline
    \quad \textbf{Quad + Constraint} & 94.59 & 84.34 & 53.56 	 & 84.34 \\
    \hline
    \end{tabular}%
  \label{tab:performance_fb15k_237_fold_1}%
\end{table}%

